Testing the Quasar Hubble Diagram with LISA Standard Sirens

Quasars have recently been used as an absolute distance indicator, extending the Hubble diagram to high redshift to reveal a deviation from the expansion history predicted for the standard, $\Lambda$CDM cosmology. Here we show that the Laser Interferometer Space Antenna (LISA) will efficiently test this claim with standard sirens at high redshift, defined by the coincident gravitational wave (GW) and electromagnetic (EM) observations of the merger of massive black hole binaries (MBHBs). Assuming a fiducial $\Lambda$CDM cosmology for generating mock standard siren datasets, the evidence for the $\Lambda$CDM model with respect to an alternative model inferred from quasar data is investigated. By simulating many realizations of possible future LISA observations, we find that for $50\%$ of these realizations (median result) 4 MBHB standard siren measurements will suffice to strongly differentiate between the two models, while 14 standard sirens will yield a similar result in $95\%$ of the realizations. In addition, we investigate the measurement precision of cosmological parameters as a function of the number of observed LISA MBHB standard sirens, finding that 15 events will on average achieve a relative precision of 5\% for $H_0$, reducing to 3\% and 2\% with 25 and 40 events, respectively. Our investigation clearly highlights the potential of LISA as a cosmological probe able to accurately map the expansion of the universe at $z\gtrsim 2$, and as a tool to cross-check and cross-validate cosmological EM measurements with complementary GW observations.

==> RefereeResponse.tex <==
To the Editors,

We thank the referee for the very useful report. We have carefully worked through the suggestions and comments, itemized below, and made revisions to the text as noted. We hope that the manuscript now addresses all concerns and questions, and is suitable for publication.

Sincerely,

L. Speri 
N. Tamanini
R. Caldwell
J. Gair
B. Wang


----------------------------------------------------------------------
Report of the Referee -- DX12732/Speri
----------------------------------------------------------------------

Please accept my apologies for my delayed response. The paper on
"Testing the Quasar Hubble Diagram with LISA Standard Sirens" by L.
Speri et al explores the interesting possibility of testing the quasar
Hubble diagram with LISA measurements at z>2, a regime that is
currently not reached by dedicated cosmological surveys to date. The
paper is worth publishing in some form, and I would be very positive
about it. However, I have some criticisms to raise here:

>> 1) By the time LISA flies (2030s), the quasar Hubble diagram will likely have been explored and constrained in much more detail then what is presented here. For instance, one possibility is that there might not be any discrepancy at high redshift after all. Also, the cosmological constraints from quasars might overshadow LISA, even at high redshift. The paper shows that LISA can constrains a deviation from LCDM to better precision with larger and larger number of events, which is fine. However nothing is said about the expected number of quasars usable for Hubble diagram analysis in the 2030s, so it looks like comparing current quasar measurements with future measurements in more than a decade from now. Interesting, but not very realistic or competitive.

Response:
We have added a discussion in the introduction about the likely state of the quasar Hubble diagram by the time LISA flies. Some estimates suggest the data set could grow by a factor of 10, and extend to as deep a redshift as LISA reaches.  However, we emphasize that the number of objects in the catalog is not the limiting factor. Rather, the major barrier is the scatter in the X-ray and UV relationship and any underlying systematic effects. Time will tell if the quasar Hubble diagram can be refined, and whether the discrepancy with the LCDM expansion history persists. We have pointed this out in the Introduction (next to last paragraph), as well as the Discussion (first paragraph).
 


>> 2) As above, the authors do not contextualise their analysis in light of the expected performance of galaxy surveys, e.g. Euclid and LSST, or redshift surveys. By the 2030s any "tension" might have been resolved, or be completely different from what is now. Surely reaching z>2 will prove a bit tricky for galaxy surveys, probably easier with quasars or AGNs. How LISA can really contribute to this picture? Surely, it sounds a bit diminishing for LISA to “just” test the present quasar diagram.

Response:
Thanks for making this point. We don't mean for LISA to take a back seat to quasars! We tried to make clear that we are simply using the quasars as a target or reference, against which we can measure the efficacy of LISA standard sirens. In response, we made changes in the Introduction (next to last paragraph) as well as the last paragraph of the Discussion/Conclusion section.
 


>> 3) Regarding Sec. II, it is not clear what is new here, and what is just taken from the literature. If it is an overview of published results/methods, this could be significantly shortened. The new elements should clearly stated.

Response:
Thanks for the suggestion. We shorted the section, but we have retained some basic material, as this may be new to a cosmology or gravitational wave reader.
 


4) Sec. III sounds a bit disconnected from the earlier discussion, and
quite a big jump for the reader. It contains a lot of methodological
material to construct catalogues/simulated data that is required for
the analysis later on, but probably not very essential for the reader.
I would suggest significantly shortening it, and move the details to
the appendix.

Response:
Again, thanks for the very useful suggestion. We significantly shortened Sec. III and moved all details to the appendix, as suggested by the referee.



5) The discussion on the Bayes factor could as well be significantly
shortened. Most of it is well known and methodological after all,
including the dependence on the prior and the difficulty of setting
thresholds (e.g. “strongly favoured”). I would focus more on the
application and results.

Response:
We removed many well known comments and we kept the essential methodology and notation for the discussion of the results. We also introduced in the result section the fact that due to the general implementation of this hypothesis testing, our code can be used to test different cosmological models with standard sirens. We expanded the captions of figures 8 and 9.



MINOR COMMENTS

>> I have included some (minor) comments on the first part up to Sec II. I will probably look into providing more detailed comments on the other sections after revision.



>> A - no citation in abstract

Response:
We removed the citation in the abstract.



>> B - references not in citation order

Response:
References are now in order of appearance.



>> C - "(CMB) [12], can retrieve information on the cosmic expansion at higher redshift, but they assume a cosmological model" I am not sure about this. H0 is directly inferred via angular diameter distance measures.

Response:
The CMB measures the angular size of the sound horizon at recombination. To extract cosmological parameters, it is necessary to supply a theoretical model of the sound horizon and the angular diameter distance D_A, which depends on the assumed expansion history. In this way, for example, the Hubble constant inferred from the CMB is model dependent.



>> D - "the Hubble constant is a nuisance parameter until the magnitude offset is known" Perhaps it is better to say they are totally degenerate

Response:
We rephrased the sentence.



>> E - "we perform a combined analysis of quasars with the SDSS-II/SNLS3 Joint Light-Curve Analysis (JLA) type Ia SNe data set" Is it the first analysis of this type?

Response:
Clarified that we are following a standard recipe and provided a reference.



>> F - "Fig. 1 shows that the LCDM model does not provide a good fit to the high redshift data, as the binned quasar measurements depart from the LCDM prediction at high redshifts." I think this statement is missing a detailed discussion of the systematic errors affecting quasar measurement as a possible explanation for the discrepancy. For instance, the same is sparse, so I suspect selection bias kicking in.

Response: It is beyond the scope of this article to delve into the possible systematics that affect the quasar sample. However, we are well aware of these possibilities. We revised the text to make clear to the reader that there may be systematic effects contaminating the data and thereby affecting the conclusions. We also refer to some recent analyses addressing these issues. We also include a comment warning of possible systematics in the next to last paragraph of section II.



>> G - "To quantify this tension, an alternative (ALT) phenomenological model of the luminosity distance is introduced" Justify this choice, it sounds like a model picked at random

Response:
This is the model used by Risaliti & Lusso. We changed the sentence to make this clear.



>>  H - "The prior on a2, a3 is chosen to be a multivariate normal distribution" Despite ALT being phenomenological, how can the priors on a2 and a3 be chosen to be Gaussian, hence informative?

Response:
We checked that the MCMC reproduces the same results also with flat priors. Therefore, we updated the respective figure using flat priors and commented in the text.
